Hierarchical Loss And Geometric Mask Refinement For Multilabel Ribs Segmentation

Automatic ribs segmentation and numeration can increase computed tomography assessment speed and reduce radiologists mistakes. We introduce a model for multilabel ribs segmentation with hierarchical loss function, which enable to improve multilabel segmentation quality. Also we propose postprocessing technique to further increase labeling quality. Our model achieved new state-of-the-art 98.2% label accuracy on public RibSeg v2 dataset, surpassing previous result by 6.7%.

==> content/03_table.tex <==
\setlength{\tabcolsep}{3pt} 
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
& \textbf{1} & \textbf{2-5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} & \textbf{11} & \textbf{12} \\
\hline
\textbf{Our*} & 98.4 & ~99.5 & 98.4 & 97.4 & 96.1 & 94.8 & 90.0 & 87.9 & 90.6 \\
\hline
\textbf{+Proc} & 98.4 & ~99.5 & 99.0 & 99.0 & 99.0 & 98.4 & 98.1 & 95.1 & 90.9 \\
\hline
\textbf{Gain} & 0.0 & 0.0 & \textcolor{green}{0.6} & \textcolor{green}{1.6} & \textcolor{green}{2.9} & \textcolor{green}{3.6} & \textcolor{green}{8.1} & \textcolor{green}{7.2} & \textcolor{green}{0.3} \\
\hline
\end{tabular}
\caption{TRSH 03: Comparison of Our* and Our+Proc* with Gain}
\label{table:comparison}
\end{table}

==> content/discussion.tex <==
\section{Discussion}
\todo{Sticky components are bad. You should not use post-processing when components are clearly stuck together.Mb describe it in conclusion?}.

